Statistical Barriers to Affine-equivariant Estimation

We investigate the quantitative performance of affine-equivariant estimators for robust mean estimation. As a natural stability requirement, the construction of such affine-equivariant estimators has been extensively studied in the statistics literature. We quantitatively evaluate these estimators under two outlier models which have been the subject of much recent work: the heavy-tailed and adversarial corruption settings. We establish lower bounds which show that affine-equivariance induces a strict degradation in recovery error with quantitative rates degrading by a factor of $\sqrt{d}$ in both settings. We find that classical estimators such as the Tukey median (Tukey '75) and Stahel-Donoho estimator (Stahel '81 and Donoho '82) are either quantitatively sub-optimal even within the class of affine-equivariant estimators or lack any quantitative guarantees. On the other hand, recent estimators with strong quantitative guarantees are not affine-equivariant or require additional distributional assumptions to achieve it. We remedy this by constructing a new affine-equivariant estimator which nearly matches our lower bound. Our estimator is based on a novel notion of a high-dimensional median which may be of independent interest. Notably, our results are applicable more broadly to any estimator whose performance is evaluated in the Mahalanobis norm which, for affine-equivariant estimators, corresponds to an evaluation in Euclidean norm on isotropic distributions.

==> content/mean_concentration.tex <==
%!TEX root = main.tex
\section{Analyzing Relaxation}
\label{sec:ept}

We first show that the optimal value of the semidefinite program \ref{eq:mt} satisfies a bounded-difference condition with respect to the $Z_i$'s.

\begin{lemma}
  \label{lem:conc}
  Let $\bm{Y} = (Y_1, \dots, Y_k)$ be any set of $k$ vectors in $\mb{R}^d$. Now, let $\bm{Y}^\prime = (Y_1, \dots, Y_i^\prime, \dots, Y_k)$ be the same set of $k$ vectors with the $i^{th}$ vector replaced by $Y_i^\prime\in \mb{R}^d$. If $m$ and $m^\prime$ are the optimal values of $\mt(x,r,\bm{Y})$ and $\mt(x,r,\bm{Y}^\prime)$, we have:
  \begin{equation*}
    \abs{m - m^\prime} \leq 1.
  \end{equation*}
\end{lemma}

\begin{proof}
  First, assume that $X$ is a feasible solution to $\mt(x,r,\bm{Y})$. Let us define $X^\prime$ as:
  \begin{equation*}
    X^\prime_{i,j} = \begin{cases}
                      X_{i,j} & \text{ if $i,j \neq b_i$} \\
                      0 &\text{otherwise}.
                     \end{cases}
  \end{equation*}
  That is, $X^\prime$ is equal to $X$ except with the row and column corresponding to $b_i$ being set to $0$. We see that $X^\prime$ forms a feasible solution to $\mt(x,r,\bm{Y}^\prime)$. Therefore, we have that:
  \begin{equation*}
    \sum_{j = 1}^k X_{b_j, b_j} = \sum_{j = 1, j\neq i}^k X^\prime_{b_j, b_j} + X_{b_i, b_i} \leq \sum_{j = 1, j\neq i}^k X^\prime_{b_j, b_j} + 1 \leq m^\prime + 1,
  \end{equation*}
where the bound $X_{b_i,b_i} \leq 1$ follows from the fact that the $2\times 2$ submatrix of $X$ formed by the rows and columns indexed by $1$ and $b_i$ is positive semidefinite and from the constraint that $X_{b_i, b_i} = X_{1, b_i}$. Since the series of equalities holds for all feasible solutions $X$ of $\mt(x,r,\bm{Y})$, we get:
  \begin{equation*}
    m \leq m^\prime + 1.
  \end{equation*}
  Through a similar argument, we also conclude that $m^\prime \leq m + 1$. Putting the two inequalities together, we obtain the required conclusion.
\end{proof}
For the next few lemmas, we are concerned with the case where $x = \mu$. Since we already know that the optimal SDP value satisfies the bounded differences condition, we need to verify that the expectation is small. As a first step towards this, we define the 2-to-1 norm of a matrix $M$.

\begin{definition}
  The 2-to-1 norm of $M \in \mb{R}^{n \times d}$ is defined as
  \begin{equation*}
    \normtto{M} = \max_{\substack{\norm{v} = 1 \\ \sigma_i \in \{\pm 1\}}} \sigma^\top M v = \max_{\norm{v} = 1} \norm{Mv}_1.
  \end{equation*}
\end{definition}
We consider the classical semidefinite programming relaxation of the 2-to-1 norm. To start with, we will define a matrix $X \in \mb{R}^{(n + d + 1) \times (n + d + 1)}$ with the rows and columns indexed by $1$ and the elements $\sigma_i$ and $v_j$. The semidefinite programming relaxation is defined as follows:
\begin{gather*}
  \max \sum_{i, j} M_{i,j} X_{\sigma_i, v_j} \\
  \text{s.t } X_{1,1} = 1,\ \sum_{j = 1}^d X_{v_j,v_j} = 1,\ X_{\sigma_i,\sigma_i} = 1,\ X \succcurlyeq 0. \tag{TOR} \label{eq:tor}
\end{gather*}
We now state a theorem of Nesterov as stated in \cite{hopkins2018sub}:
\begin{theorem}{(\cite{nesterov1998semidefinite})}
  \label{thm:contr}
  There is a constant $K_{2\rightarrow 1} = \sqrt{\pi/2} \leq 2$ such that the optimal value, $m$, of the semidefinite programming relaxation~\ref{eq:tor} satisfies:
  \begin{equation*}
    m \leq K_{2\rightarrow 1} \normtto{M}.
  \end{equation*}
\end{theorem}
In the next step, we bound the expected 2-to-1 norm of the random matrix $Z$. To do this, we begin by recalling the Ledoux-Talagrand Contraction Theorem \cite{ledoux1991probability}.
\begin{theorem}
  \label{thm:ledtal}
  Let $X_1, \dots, X_n \in \mb{R}^d$ be i.i.d.~random vectors, $\mathcal{F}$ be a class of real-valued functions on $\mb{R}^d$ and $\sigma_i, \dots, \sigma_n$ be independent Rademacher random variables. If $\phi: \mb{R} \rightarrow \mb{R}$ is an $L$-Lipschitz function with $\phi(0) = 0$, then:
  \begin{equation*}
    \mathbb{E} \sup_{f \in \mathcal{F}} \sum_{i = 1}^n \sigma_i \phi(f(X_i)) \leq L\cdot \mb{E} \sup_{f \in \mathcal{F}} \sum_{i = 1}^{n} \sigma_i f(X_i).
  \end{equation*}
\end{theorem}

We are now ready to bound the expected 2-to-1 norm of the random matrix $Z$.
\begin{lemma}
  \label{lem:tto}
  Let $\bm{Y} = (Y_1, \dots, Y_n) \in \mb{R}^{n\times d}$ be a set of $n$ i.i.d.~random vectors such that $\mb{E} [Y_i] = 0$ and $\mb{E} [Y_i Y_i^\top] = \Lambda$ and assume that:
  \begin{equation*}
      \max_{v \in \mc{S}^{d - 1}} \mb{E} \lsrs{\abs*{\inp{v}{Y}}^{1 + \alpha}} \leq \beta.
  \end{equation*}
  Then we have:
  \begin{equation*}
    \mb{E} \normtto{\bm{Y}} \leq 2 \sqrt{n\Tr \Lambda} + n \beta^{\frac{1}{1 + \alpha}}.
  \end{equation*}
\end{lemma}
\begin{proof}
  Denoting by $Y$ and $Y_i^\prime$ random vectors that are independently and identically distributed as $Y_i$ and by $\sigma_i$ independent Rademacher random variables, we have: 
  \begin{align*}
    \mb{E} [\normtto{\bm{Y}}] &= \mb{E} \lsrs{\max_{\norm{v} = 1}\sum_{i = 1}^n \abs{\inp{Y_i}{v}}} = \mb{E} \lsrs{\max_{\norm{v} = 1}\sum_{i = 1}^n \abs{\inp{Y_i}{v}} + \mb{E} \abs{\inp{v}{Y_i}} - \mb{E} \abs{\inp{v}{Y_i}}}\\
    &\leq \mb{E} \lsrs{\max_{\norm{v} = 1} \sum_{i = 1}^n \abs{\inp{Y_i}{v}} - \mb{E} \abs{\inp{Y_i^\prime}{v}}} + n \max_{\norm{v} = 1}\mb{E} [\abs{\inp{v}{Y}}] \\
    &\leq \mb{E} \lsrs{\max_{\norm{v} = 1} \sum_{i = 1}^n \sigma_i (\abs{\inp{Y_i}{v}} - \abs{\inp{Y_i^\prime}{v}})} + n \max_{\norm{v} = 1} \mb{E} \lsrs{\abs{\inp{v}{Y}}}.
  \end{align*}
  Now, we have for the second term:
  \begin{equation*}
    \max_{\norm{v} = 1}\mb{E} [\abs{\inp{v}{Y}}] \leq \max_{\norm{v} = 1} \lprp{\mb{E} \inp{v}{Y}^{1 + \alpha}}^{\frac{1}{1 + \alpha}} \leq \beta^{\frac{1}{1 + \alpha}}.
  \end{equation*}
  For the first term, we employ a standard symmetrization argument:
  \begin{align*}
    \mb{E} \lsrs{\max_{\norm{v} = 1} \sum_{i = 1}^n \sigma_i (\abs{\inp{Y_i}{v}} - \abs{\inp{Y_i^\prime}{v}})} & \leq \mb{E} \lsrs{\max_{\norm{v} = 1} \sum_{i = 1}^n \sigma_i \abs{\inp{Y_i}{v}}} + \mb{E}\lsrs{\max_{\norm{v} = 1}\sum_{i = 1}^n-\sigma_i\abs{\inp{Y_i^\prime}{v}}} \\
    &= 2 \mb{E} \lsrs{\max_{\norm{v} = 1} \sum_{i = 1}^n \sigma_i\abs{\inp{v}{Y_i}}} \leq 2 \mb{E} \lsrs{\max_{\norm{v} = 1} \sum_{i = 1}^n \sigma_i\inp{v}{Y_i}} \\
    &= 2 \mb{E} \lsrs{\norm*{\sum_{i = 1}^n \sigma_i Y_i}} \leq 2 \lprp{\mb{E} \lsrs{\norm*{\sum_{i = 1}^n \sigma_i Y_i}^2}}^{1/2} \\
    &= 2 \lprp{\mb{E} \sum_{1 \leq i,j \leq n} \sigma_i \sigma_j \inp{Y_i}{Y_j}}^{1/2} = 2\sqrt{n\Tr \Lambda},
  \end{align*}
  where the second inequality follows from the Ledoux-Talagrand Contraction Principle (Theorem~\ref{thm:ledtal}).
  By putting these two bounds together, we prove the lemma.
\end{proof}

We now bound the expected value of $\mt(\mu,r,\bm{Y})$ by relating it to $\normtto{\bm{Y}}$.
\begin{lemma}
  \label{lem:exp}
  Let $\bm{Y} = (Y_1, \dots, Y_k) \in \mb{R}^{k\times d}$ be a collection of $k$ i.i.d.~random vectors with mean $\mu$ and covariance $\Lambda$ and assume that:
  \begin{equation*}
      \max_{v \in \mc{S}^{d - 1}} \mb{E} \lsrs{\abs*{\inp{v}{Y}}^{1 + \alpha}} \leq \beta.
  \end{equation*} 
  Denoting by $\mathcal{S}$ the set of feasible solutions for $\mt(\mu,r,\bm{Y})$, we have:
  \begin{equation*}
    \mb{E} \max_{x \in \mathcal{S}} \sum_{i = 1}^k X_{1, b_i} \leq \frac{1}{2r} \lprp{5 \sqrt{k \Tr \Lambda} + 2k \beta^{\frac{1}{1 + \alpha}}}.
  \end{equation*}
\end{lemma}

\begin{proof}
  First, let $X$ be a feasible solution for $\mt(\mu, r, \bm{Y})$. We construct a new matrix $W$ which is indexed by $\sigma_i$ and $v_j$ as opposed to $b_i$ and $v_j$ for $X$:
  \begin{gather*}
    W_{\sigma_i, \sigma_j} = 4X_{b_i, b_j} - 2 X_{1, b_i} - 2 X_{1, b_j} + 1,\quad W_{v_i, v_j} = X_{v_i, v_j},\quad W_{1,1} = 1, \\
    W_{1, v_i} = X_{1, v_i}, \quad W_{1, \sigma_i} = 2X_{1, b_i} - 1, \quad W_{v_i, \sigma_j} = 2X_{v_i, b_j} - X_{1, v_i}.
  \end{gather*}
  We prove that $W$ is a feasible solution to the SDP relaxation~\ref{eq:tor} of $\bm{Y} - \mu$. We see that:
  \begin{equation*}
    W_{\sigma_i, \sigma_i} = 1 \text{ and } \sum_{i = 1}^{d} W_{v_i, v_i} = 1.
  \end{equation*}
  Thus, we simply need to verify that $W$ is positive semidefinite. Let $w \in \mb{R}^{k + d + 1}$ be indexed by $1$, $\sigma_i$ and $v_j$. We construct from $w$ a new vector $w^\prime$, indexed by $1$, $b_i$ and $v_j$ and defined as follows:
  \begin{equation*}
    w^\prime_{1} = w_{1} - \sum_{i = 1}^k w_{\sigma_i}, \quad w^\prime_{b_i} = 2 w_{\sigma_i}, \quad w^\prime_{v_j} = w_{v_j}.
  \end{equation*}
  With $w^\prime$ defined in this way, we have the following equality:
  \begin{equation*}
    w^\top W w = (w^\prime)^\top X w^\prime \geq 0.
  \end{equation*}
  Since the condition holds for all $w \in \mb{R}^{k + d + 1}$, we get that $W \succcurlyeq 0$. Therefore, we conclude that $W$ is a feasible solution to the SDP relaxation~\ref{eq:tor} of $\bm{Y} - \mu$.

  We bound the expected value of $\mt(\mu,r,\bm{Y})$ as follows, denoting by $v_{b_i}$ the vector $(X_{b_i, v_1}, \dots, X_{b_i, v_d})$ and by $v$ the vector $(X_{1, v_1}, \dots, X_{1, v_d})$:
  \begin{align*}
    \mb{E} \max_{X \in \mathcal{S}} \sum_{i = 1}^k X_{1, b_i} &= \mb{E} \max_{X \in \mathcal{S}} \sum_{i = 1}^k X_{b_i, b_i} \leq \frac{1}{r}\mb{E} \max_{X \in \mathcal{S}} \sum_{i = 1}^k \inp{v_{b_i}}{Y_i - \mu} \\
    &= \frac{1}{2r} \mb{E} \max_{X \in S}\Big[ \sum_{i = 1}^k \inp{2v_{b_i} - v}{Y_i - \mu} + \sum_{i = 1}^k \inp{v}{Y_i - \mu}\Big] \\
    &\leq \frac{1}{2r} \lprp{\mb{E} \max_{X \in S} \sum_{i = 1}^k \inp{2v_{b_i} - v}{Y_i - \mu} + \mb{E} \max_{X \in \mathcal{S}} \sum_{i = 1}^k \inp{v}{Y_i - \mu}}.
  \end{align*}
  From the fact that $X$ is positive semidefinite, and from the fact that the $2\times 2$ submatrix indexed by $v_i$ and $b_j$ is positive semidefinite, we obtain:
  \begin{equation*}
    X^2_{v_i,b_j} \leq X_{v_i, v_i} X_{b_j, b_j} \leq X_{v_i, v_i} \implies \norm{v_{b_j}}^2= \sum_{i = 1}^d X^2_{v_i, b_j}  \leq \sum_{i = 1}^d X_{v_i, v_i} = 1.
  \end{equation*}
  Therefore, we get for the second term in the above equation:
  \begin{equation*}
    \mb{E} \max_{X \in \mathcal{S}} \sum_{i = 1}^{k} \inp{v}{Y_i - \mu} \leq \mb{E} \norm*{\sum_{i = 1}^{k} Y_i - \mu} \leq \lprp{\mb{E} \norm*{\sum_{i = 1}^{k} Y_i - \mu}^2}^{1/2} = (k \Tr \Lambda)^{1/2}.
  \end{equation*}
  We bound the first term using the following series of inequalities where $W$ is constructed from $X$ as described above:
  \begin{align*}
    \mb{E} \max_{x \in \mathcal{S}} \sum_{i = 1}^k \inp{2v_{b_i} - v}{Y_i - \mu} &= \mb{E} \max_{x \in \mathcal{S}} \sum_{i = 1}^k \sum_{j = 1}^d (Y_i - \mu)_j W_{\sigma_i, v_j} = \mb{E} \max_{x \in \mathcal{S}} \sum_{i = 1}^k \sum_{j = 1}^d (\bm{Y}_{i, j} - \mu_j) W_{\sigma_i, v_j} \\
    &\leq 2 \mb{E} \normtto{\bm{Y} - \bm{1}\mu^\top} \leq 4 \sqrt{k \Tr \Lambda} + 2 k \beta^{\frac{1}{1 + \alpha}},
  \end{align*}
  where the first inequality follows from Theorem~\ref{thm:contr} and the second inequality follows from Lemma~\ref{lem:tto}. By combining these three inequalities, we get:
  \begin{equation*}
    \mb{E} \max_{x \in \mathcal{S}} \sum_{i = 1}^k X_{1, b_i} \leq \frac{1}{2r} \lprp{5 \sqrt{k \Tr \Lambda} + 2 k \beta^{\frac{1}{1 + \alpha}}}.
  \end{equation*}
\end{proof}  

Finally, we establish the main technical result of this section, \cref{lem:rst_bound}.

\begin{proof}[Proof of \cref{lem:rst_bound}]
  From \cref{lem:exp}, we see that:
  \begin{equation*}
    \mb{E} \max_{X \in \mathcal{S}} \sum_{i = 1}^k X_{b_i, b_i} \leq \frac{k}{40}.
  \end{equation*}
  Now from \cref{lem:conc} and an application of the bounded difference inequality (see, for example, Theorem~6.2 in \cite{boucheron2013concentration}), with probability at least $1 - e^{k / 800}$:
  \begin{equation*}
    \max_{X \in \mathcal{S}} \sum_{i = 1}^k X_{b_i, b_i} \leq \frac{k}{20}.
  \end{equation*}
\end{proof}

In the following lemma, we analyze the set of random vectors returned by \cref{alg:part}. It will be useful to condition on the conclusion of \cref{lem:init}.

\begin{lemma}
  \label{lem:part}
  Let $\bm{X} = \{X_i\}_{i = 1}^n \ts \nu$ be iid zero-mean random vectors, satisfying the weak-moment condition for some $\alpha > 0$. Furthermore, suppose $x^\dagger$ satisfies $\norm{x^\dagger} \leq 24\sqrt{d}$. Then, the set of vectors $\bm{Y}$ returned by \cref{alg:part} with input $\bm{X}$ and $x^\dagger$ are iid random vectors vectors with mean $\tld{\mu}$ and covariance $\tld{\Sigma}$ and satisfy:
  \begin{gather*}
    \text{Claim 1: } \mb{P} \lbrb{\abs{\bm{Y}} \geq \frac{3n}{4}} \geq 1 - e^{- \frac{n}{50}}, \qquad \qquad \text{Claim 2: } \norm{\tld{\mu}} \leq 2 \lprp{\frac{d}{n}}^{\frac{\alpha}{1 + \alpha}} \\
    \text{Claim 3: } \forall \norm{v} = 1:\mb{E} \lsrs{\abs*{\inp{Y_i - \tld{\mu}}{v}}^{1 + \alpha}} \leq 20,\qquad\text{Claim 4: } \tr \tld{\Sigma} \leq 750 \max \lprp{n^{\frac{1 - \alpha}{1 + \alpha}}d^{\frac{2\alpha}{(1 + \alpha)}}, d}.
  \end{gather*}
\end{lemma}

\begin{proof}
  First, consider the set $A = \{x: \norm{x - x^\dagger} \leq \thr\}$ as defined in \cref{alg:part}. Note from the definition of the set $A$ that $\{x: \norm{x} \leq 0.75\thr\} \subseteq A$. We have from Markov's inequality and \cref{lem:lmom}:
  \begin{equation*}
    \mb{P} \lbrb{X_i \in A} \geq 1 - \min \lprp{\frac{d}{n}, \frac{1}{25}}
  \end{equation*}
  Therefore, by an application of Hoeffding's inequality, using the definition of the set of points $Y_1, \dots, Y_m$, we have that, with probability at least $1 - e^{- \frac{n}{50}}$:
  \begin{equation*}
    \abs{\bm{Y}} \geq \frac{3n}{4}
  \end{equation*}
  This proves the first claim of the lemma. For the next two claims, note that conditioned on the random variable $\hat{\mu}$, each of the $Y_i$ are independent and identically distributed according to $\nu_{A}$. Again, we get from the bound on $\mb{P} \lbrb{X_i \in A}$ by an application of \cref{lem:mnshft}, the next two claims of the lemma:
  \begin{equation*}
    \text{Claim 2: } \norm{\tld{\mu}} \leq 2 \lprp{\frac{d}{n}}^{\frac{\alpha}{1 + \alpha}}, \qquad \text{Claim 3: }\forall \norm{v} = 1:\mb{E} \lsrs{\abs*{\inp{Y_i - \tld{\mu}}{v}}^{1 + \alpha}} \leq 20.
  \end{equation*}
  For the final claim, note that as $\norm{x^\dagger} \leq 24 \sqrt{d}$, we have $A \subseteq B \coloneqq \lbrb{x: \norm{x} \leq 1.25\tau}$. Therefore, we have by the property of the mean that:
  \begin{align*}
    \tr \tld{\Sigma} = \mb{E} \lsrs{\norm{Y_i - \tld{\mu}}^2} &\leq \mb{E} \lsrs{\norm{Y_i}^2} = \frac{1}{\nu(A)} \mb{E} \lsrs{\norm{X_j}^2 \bm{1} \{X_j \in A\}} \\ 
    &\leq 2 \mb{E} \lsrs{\norm{X_j}^2 \bm{1} \{X_j \in B\}} \leq 750 \max \lprp{n^{\frac{1 - \alpha}{1 + \alpha}}d^{\frac{2\alpha}{(1 + \alpha)}}, d},
  \end{align*}
  where the final inequality follows from \cref{lem:trsig} and the definition of $\thr$.
\end{proof}

The main result of this section is the following high probability guarantee on the set of points output by \cref{alg:loce}.
\begin{lemma}
\label{lem:mnConc}
Let $\delta > e^{n / 8000}$ and $\bm{X} = \{X_i\}_{i = 1}^n$ be iid random vectors with mean $\mu$, satisfying the weak-moment condition for some known $\alpha > 0$. Furthermore, suppose that $x^\dagger$ satisfies $\norm{x^\dagger - \mu} \leq 24 \sqrt{d}$. Let $\bm{Z} = \{Z_i\}_{i = 1}^k$ denote the set of vectors output by \cref{alg:loce} run with inputs $\bm{X}$, $x^\dagger$ and $\delta$. Then, there exists a point $\tld{\mu}$ such that for all $r \geq \rad$:
\begin{equation*}
  \norm{\tld{\mu} - \mu} \leq 2 \lprp{\frac{d}{n}}^{\frac{\alpha}{1 + \alpha}}\text{ and } \max_{X \in \mathcal{S}} \sum_{i = 1}^k X_{b_i, b_i} \leq \frac{k}{20},
\end{equation*}
with probability at least $1 - \delta / 2$ where $\mathcal{S}$ denotes the set of feasible solutions of $\ref{eq:mt}(\tld{\mu}, r, \bm{Z})$.
\end{lemma}

\begin{proof}
  Note that it is sufficient to prove the lemma in the specific case where $\mu = \bm{0}$. We may now assume each of the $Y_i$ are iid random variables satisfying the conclusions of \cref{lem:part}. Therefore, $Z_i$ are iid random vectors with mean $\tld{\mu}$ and  covariance $\tld{\Sigma}$ satisfying:
  \begin{equation*}
    \norm{\tld{\mu}} \leq 2 \lprp{\frac{d}{n}}^{\frac{\alpha}{1 + \alpha}}\qquad \tr \tld{\Sigma} \leq \frac{750 k\max \lprp{n^{\frac{1 - \alpha}{1 + \alpha}}d^{\frac{2\alpha}{(1 + \alpha)}}, d}}{n}.
  \end{equation*}
  Furthermore, we have by an application of \cref{lem:srv} that:
  \begin{equation*}
    \forall \norm{v} = 1: \mb{E} \lsrs{\abs*{\inp{v}{Z_i - \tld{\mu}}}^{1 + \alpha}} \leq 80 \lprp{\frac{k}{n}}^{\alpha}.
  \end{equation*}
  Finally, the conclusion of the lemma follows by an application of \cref{lem:rst_bound} and the bound on the probabilities follows from the bounds in \cref{lem:rst_bound,lem:part}.
\end{proof}
